ModSelect: Automatic Modality Selection for Synthetic-to-Real Domain Generalization

Modality selection is an important step when designing multimodal systems, especially in the case of cross-domain activity recognition as certain modalities are more robust to domain shift than others. However, selecting only the modalities which have a positive contribution requires a systematic approach. We tackle this problem by proposing an unsupervised modality selection method (ModSelect), which does not require any ground-truth labels. We determine the correlation between the predictions of multiple unimodal classifiers and the domain discrepancy between their embeddings. Then, we systematically compute modality selection thresholds, which select only modalities with a high correlation and low domain discrepancy. We show in our experiments that our method ModSelect chooses only modalities with positive contributions and consistently improves the performance on a Synthetic-to-Real domain adaptation benchmark, narrowing the domain gap.

==> misc/class_examples.tex <==
\begin{figure*}[h]
    \centering % <-- added
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/class_examples/sims_cook.png}
  \caption{Sims4Action Cook}
  \label{fig:baseline_1}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/class_examples/sims_watch_tv.png}
    \caption{Sims4Action Watch TV}

  \label{fig:baseline_2}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/class_examples/sims_eat.png}
    \caption{Sims4Action Eat}

  \label{fig:baseline_3}
\end{subfigure}

%
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/class_examples/toyota_cook.png}
    \caption{Toyota Cook}

  \label{fig:4}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/class_examples/toyota_watch_tv.png}
    \caption{Toyota Watch TV}

  \label{fig:baseline_5}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/class_examples/toyota_eat.png}
    \caption{Toyota Eat}

  \label{fig:baseline_6}
\end{subfigure}

\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/class_examples/etri_cook.png}
    \caption{ETRI Cook}

  \label{fig:4}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/class_examples/etri_watch_tv.png}
    \caption{ETRI Watch TV}

  \label{fig:baseline_5}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/class_examples/etri_eat.png}
    \caption{ETRI Eat}

  \label{fig:baseline_6}
\end{subfigure}
\caption{Example images for the Cook, Watch TV, and Eat classes from the three datasets.}
       \Description{Figure 10. Fully described in the text.}
\label{fig:example_classes}
\end{figure*}



==> sections/image_examples.tex <==
\section{Image Examples from All Datasets}

Figure~\ref{fig:example_classes} shows example images from all three datasets for the Cook, Watch TV and Drink action classes. Our experiments show a smaller \textsc{Synthetic$\rightarrow$Real} domain gap to Toyota~\cite{das2019toyota} than to ETRI~\cite{jang2020etri}. This could be explained by the large difference in viewpoints, which in Sims4Action~\cite{roitberg2021let} and Toyota are mostly from the top, whereas in ETRI are taken from lower angles. The furniture in Sims4Action is designed to mimic the household setting in Toyota, e.g., sofa with a coffee table and TV in the living room and large table in the dining room. In ETRI, we can see that there is a large difference in the furnishing, e.g. the subject is not sitting on a sofa when watching TV and the dining table is positioned against a wall. 

The YOLO modality shows the best domain generalization out of all of the modalities. We hypothesize that this might be caused by its simplicity and \textbf{abstraction} from the concrete details of the scene, e.g. whether the person is sitting on the floor while watching TV or on a sofa or if the table is positioned one way or another. Additionally, the viewpoint angles do not play a role in the detections representation \textbf{v}, which makes YOLO even more robust to domain shift.

==> sections/notation_table.tex <==
\section{Notation Table}
\label{sec:notation_table}
The notation Table \ref{tab:notation_table} summarizes all the terms of our equations and explains them in detail. 
\input{tables/notation_table}

==> tables/action_classes.tex <==
\begin{table}[h]
    \centering
        \caption{List of all $N=10$ action classes used for training and evaluation.}
    \scalebox{0.95}{
    \begin{tabular}{cc}
    \toprule
        Cook &
        Drink \\
        Eat &
        Read Book \\
        Get up / Sit down &
        Use Computer \\
        Use Phone &
        Use Tablet \\
        Walk &
        Watch TV
         \\
        \bottomrule
    \end{tabular}}
    \label{tab:action_classes}
\end{table}

==> tables/baseline_results.tex <==
\begin{table}[h]
    \centering
    \caption{Average contribution $f(m)$ over the $6$ late fusion methods of each modality $m$. Negative contributions are colored in \color{red}{red}.}
    \label{tab:baseline_results}
    \begin{tabular}{l|c|c|c|c|c}
    \toprule
        Test Dataset & \multicolumn{5}{c}{Contribution $f(m)$} \\ \hline
         {} & H & L & OF & RGB & YOLO  \\ \hline
        Sims4Action~\cite{roitberg2021let} & 4.37 & 8.86 & \color{red}{-0.74} & 6.98 & \color{red}{-2.57} \\ 
        Toyota~\cite{das2019toyota} & 2.14 & 2.46 & 2.90 & \color{red}{-1.86} & 2.13 \\ 
        ETRI~\cite{jang2020etri} & 0.76 & 1.60 & \color{red}{-0.13} & \color{red}{-1.17} & 2.02 \\ 
        \bottomrule
    \end{tabular}
\end{table}

==> tables/correlations.tex <==
\begin{table}[b]
    \centering
    \caption{Aggregated prediction correlation $\rho(m)$ values for each modality $m$ on the three test datasets and the aggregated thresholds $\delta_{\textbf{agg}}^{\rho}$. Values \textbf{below} the threshold are colored in \color{red}{red}.}
    \label{tab:agg_correlation_results}
    \begin{tabular}{l|ccccc|c}
    \toprule
        Test Dataset & \multicolumn{5}{c|}{Aggregated Correlation $\rho(m)$} & {} \\ \hline 
        {} & H & L & OF & RGB & YOLO & $\delta_{\textbf{agg}}^{\rho}$  \\ \hline
        Sims4Action~\cite{roitberg2021let} & 0.57 & 0.55 & \color{red}{0.38} & 0.50 & \color{red}{0.37} & 0.40  \\
        Toyota~\cite{das2019toyota} & 0.23 & 0.21 & 0.14 & \color{red}{0.08} & 0.14 & 0.10 \\
        ETRI~\cite{jang2020etri} & 0.14 & 0.14 & \color{red}{0.06} & \color{red}{0.05} & 0.13 & 0.08 \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/discrepancy.tex <==
\begin{table}
    \centering
        \caption{Aggregated $MMD(m)$ values for each modality $m$ on the three test datasets and the aggregated thresholds $\delta_{\textbf{agg}}^{MMD}$. Values \textbf{above} the threshold are colored in \color{red}{red}.}
    \label{tab:agg_discrepancy_results}
    \begin{tabular}{l|cccc|c}
    \toprule
        Test Dataset & \multicolumn{4}{c|}{Aggregated Discrepancy $MMD(m)$} & {} \\ \hline 
        {} & H & L & OF & RGB & $\delta_{\textbf{agg}}^{MMD}$  \\ \hline
        Sims4Action~\cite{roitberg2021let} & 9.49 & 8.12 & \color{red}{13.07} & 9.92 & 10.15 \\
        Toyota~\cite{das2019toyota} & 11.93 & 11.47 & 13.34 & \color{red}{20.79} & 14.38 \\
        ETRI~\cite{jang2020etri} & 17.84 & 17.76 & \color{red}{22.04} & \color{red}{24.91} & 20.64 \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/ef_lf_results.tex <==
\begin{table}[]
    \centering
    \scalebox{0.75}{
    \begin{tabular}{l|cc|cc|cc}
    \toprule
        {} & \multicolumn{2}{c|}{\textsc{Synthetic}}& \multicolumn{4}{c}{\textsc{Real}} \\ \hline
        \multirow{1}{*}{\thead{\diagbox[height=2.2em]{Modalities}{Test Set}}} & \multicolumn{2}{c|}{Sims4Action~\cite{roitberg2021let}} & \multicolumn{2}{c|}{Toyota~\cite{das2019toyota}} & \multicolumn{2}{c}{ETRI~\cite{jang2020etri}} \\ \cline{2-7} 
         {} & EF & LF & EF & LF & EF & LF  \\ \hline
         H & \multicolumn{2}{c|}{$71.38$} & \multicolumn{2}{c|}{$20.23$} & \multicolumn{2}{c}{$12.12$} \\
         %
         L & \multicolumn{2}{c|}{$75.09$} & \multicolumn{2}{c|}{$22.00$} & \multicolumn{2}{c}{$12.88$} \\
         %
         OF & \multicolumn{2}{c|}{$44.50$} & \multicolumn{2}{c|}{$21.34$} & 
         \multicolumn{2}{c}{$9.28$} \\
         %
         RGB & \multicolumn{2}{c|}{$61.79$} & \multicolumn{2}{c|}{$13.74$} & 
         \multicolumn{2}{c}{$9.37$}\\
         %
         YOLO & \multicolumn{2}{c|}{$50.54$} & \multicolumn{2}{c|}{$26.08$} & \multicolumn{2}{c}{$38.25$} \\ \hline
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L & $57.84$ & $91.48$ & $15.69$ & $23.44$ & $11.98$ & $16.95$ \\
         %
         H OF & $71.14$ & $89.86$ & $16.67$ & $25.97$ & $10.07$ & $15.10$ \\
         %
         H RGB & $76.77$ & $94.44$ & $10.25$ & $21.38$ & $5.80$ & $13.91$ \\
         %
         L OF & $72.73$ & $90.84$ & $19.69$ & $25.60$ & $9.15$ & $15.90$ \\
         %
         L RGB & $81.54$ & $94.42$ & $13.47$ & $20.58$ & $10.74$ & $15.46$ \\
         %
         OF RGB & $70.40$ & $86.15$ & $19.43$ & $18.50$ & $11.68$ & $12.85$ \\ 
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H YOLO & $\sim$ & $74.86$ & $\sim$ & $25.51$ & $\sim$ & $20.55$ \\
         %
         L YOLO & $\sim$ & $80.25$ & $\sim$ & $24.77$ & $\sim$ & $19.91$ \\
         %
         OF YOLO & $\sim$ & $62.21$ & $\sim$ & $27.56$ & $\sim$ & $20.34$ \\
         %
         RGB YOLO & $\sim$ & $76.23$ & $\sim$ & $17.29$ & $\sim$ & $19.41$ \\ \hline
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L OF & $77.12$ & $94.03$ & $25.19$ & $26.70$ & $12.14$ & $17.26$ \\
         %
         H L RGB & $73.66$ & $95.72$ & $15.32$ & $23.25$ & $4.63$ & $15.78$ \\
         %
         H OF RGB & $70.70$ & $95.41$ & $11.58$ & $23.73$ & $10.24$ & $13.79$ \\
         %
         L OF RGB & $82.98$ & $95.61$ & $11.95$ & $24.09$ & $9.16$ & $15.49$ \\ 
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L YOLO & $\sim$ & $86.57$ & $\sim$ & $25.80$ & $\sim$ & $20.46$ \\
         H OF YOLO & $\sim$ & $82.97$ & $\sim$ & $29.48$ & $\sim$ & $19.91$ \\
         H RGB YOLO & $\sim$ & $88.79$ & $\sim$ & $23.27$ & $\sim$ & $17.77$ \\
         L OF YOLO & $\sim$ & $86.31$ & $\sim$ & $28.51$ & $\sim$ & $20.68$ \\
         L RGB YOLO & $\sim$ & $90.59$ & $\sim$ & $23.29$ & $\sim$ & $19.09$ \\
         OF RGB YOLO & $\sim$ & $82.37$ & $\sim$ & $21.15$ & $\sim$ & $16.92$ \\ \hline
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L OF RGB & $66.77$ & $96.95$ & $12.11$ &  $26.00$ & $8.23$ & $16.22$ \\
         %
         H L OF YOLO & $\sim$ & $90.05$ & $\sim$ & $28.98$ & $\sim$ & $20.27$ \\
         %
         H L RGB YOLO & $\sim$ & $92.88$ & $\sim$ & $25.36$ & $\sim$ & $18.55$ \\
         %
         H OF RGB YOLO & $\sim$ & $91.14$ & $\sim$ & $26.10$ & $\sim$ & $17.20$ \\
         %
         L OF RGB YOLO & $\sim$ & $92.56$ & $\sim$ & $26.12$ & $\sim$ & $18.56$ \\ \hline
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L OF RGB YOLO & $\sim$ & $94.27$ & $\sim$ & $27.52$ & $\sim$ & $18.53$ \\
         \bottomrule
    \end{tabular}}
    \caption{Results from the action classifiers trained on Sims4Action. The late fusion results are averaged over the $6$ strategies discussed in Section \ref{sec:modality_extraction_and_training}. All results are in the mPCA metric. EF and LF denote Early and Late Fusion.}
    \label{tab:ef_lf_results}
\end{table}

==> tables/if_results_transposed.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{ccccccccccccccccccccccccccccccccccc}
\cline{1-1} \cline{3-5} \cline{10-10} \cline{20-20} \cline{30-30} \cline{35-35}
\multicolumn{1}{l}{\{\}}                             & \multicolumn{1}{l}{\{\}}       & \multicolumn{1}{r|}{Test Set}                         & \multicolumn{1}{l|}{Modalities} & \multicolumn{1}{l}{H}        & \multicolumn{1}{l}{L}        & \multicolumn{1}{l}{OF}       & \multicolumn{1}{l}{RGB}      & \multicolumn{1}{l}{YOLO}     & \multicolumn{1}{l}{H L}      & \multicolumn{1}{l}{H OF}     & \multicolumn{1}{l}{H RGB}    & \multicolumn{1}{l}{L OF}     & \multicolumn{1}{l}{L RGB}    & \multicolumn{1}{l}{OF RGB}   & \multicolumn{1}{l}{H YOLO}   & \multicolumn{1}{l}{L YOLO}   & \multicolumn{1}{l}{OF YOLO}  & \multicolumn{1}{l}{RGB YOLO} & \multicolumn{1}{l}{H L OF}   & \multicolumn{1}{l}{H L RGB}  & \multicolumn{1}{l}{H OF RGB} & \multicolumn{1}{l}{L OF RGB} & \multicolumn{1}{l}{H L YOLO} & \multicolumn{1}{l}{H OF YOLO} & \multicolumn{1}{l}{H RGB YOLO} & \multicolumn{1}{l}{L OF YOLO} & \multicolumn{1}{l}{L RGB YOLO} & \multicolumn{1}{l}{OF RGB YOLO} & \multicolumn{1}{l}{H L OF RGB} & \multicolumn{1}{l}{H L OF YOLO} & \multicolumn{1}{l}{H L RGB YOLO} & \multicolumn{1}{l}{H OF RGB YOLO} & \multicolumn{1}{l}{L OF RGB YOLO} & \multicolumn{1}{l}{H L OF RGB YOLO} \\ \cline{1-5} \cline{10-10} \cline{20-20} \cline{30-30} \cline{35-35} 
\multicolumn{1}{|c|}{\multirow{3}{*}{mPCA {[}\%{]}}} & \multicolumn{1}{c|}{Synthetic} & \multicolumn{1}{c|}{Sims4Action$\sim$roitberg2021let} & \multicolumn{1}{c|}{\{\}}       & \multicolumn{1}{c|}{$71.38$} & \multicolumn{1}{c|}{$75.09$} & \multicolumn{1}{c|}{$44.50$} & \multicolumn{1}{c|}{$61.79$} & \multicolumn{1}{c|}{$50.54$} & \multicolumn{1}{c|}{$91.48$} & \multicolumn{1}{c|}{$89.86$} & \multicolumn{1}{c|}{$94.44$} & \multicolumn{1}{c|}{$90.84$} & \multicolumn{1}{c|}{$94.42$} & \multicolumn{1}{c|}{$86.15$} & \multicolumn{1}{c|}{$74.86$} & \multicolumn{1}{c|}{$80.25$} & \multicolumn{1}{c|}{$62.21$} & \multicolumn{1}{c|}{$76.23$} & \multicolumn{1}{c|}{$94.03$} & \multicolumn{1}{c|}{$95.72$} & \multicolumn{1}{c|}{$95.41$} & \multicolumn{1}{c|}{$95.61$} & \multicolumn{1}{c|}{$86.57$} & \multicolumn{1}{c|}{$82.97$}  & \multicolumn{1}{c|}{$88.79$}   & \multicolumn{1}{c|}{$86.31$}  & \multicolumn{1}{c|}{$90.59$}   & \multicolumn{1}{c|}{$82.37$}    & \multicolumn{1}{c|}{$96.95$}   & \multicolumn{1}{c|}{$90.05$}    & \multicolumn{1}{c|}{$92.88$}     & \multicolumn{1}{c|}{$91.14$}      & \multicolumn{1}{c|}{$92.56$}      & $94.27$                             \\ \cline{2-5} \cline{10-10} \cline{20-20} \cline{30-30} \cline{35-35} 
\multicolumn{1}{|c|}{}                               & \multirow{2}{*}{Real}          & Toyota$\sim$das2019toyota                             & \{\}                            & $20.23$                      & $22.00$                      & $21.34$                      & $13.74$                      & $26.08$                      & $23.44$                      & $25.97$                      & $21.38$                      & $25.60$                      & $20.58$                      & $18.50$                      & $25.51$                      & $24.77$                      & $27.56$                      & $17.29$                      & $26.70$                      & $23.25$                      & $23.73$                      & $24.09$                      & $25.80$                      & $29.48$                       & $23.27$                        & $28.51$                       & $23.29$                        & $21.15$                         & $26.00$                        & $28.98$                         & $25.36$                          & $26.10$                           & $26.12$                           & $27.52$                             \\ \cline{3-5} \cline{10-10} \cline{20-20} \cline{30-30} \cline{35-35} 
\multicolumn{1}{|c|}{}                               &                                & ETRI$\sim$jang2020etri                                & \{\}                            & $12.12$                      & $12.88$                      & $9.28$                       & $9.37$                       & $38.25$                      & $16.95$                      & $15.10$                      & $13.91$                      & $15.90$                      & $15.46$                      & $12.85$                      & $20.55$                      & $19.91$                      & $20.34$                      & $19.41$                      & $17.26$                      & $15.78$                      & $13.79$                      & $15.49$                      & $20.46$                      & $19.91$                       & $17.77$                        & $20.68$                       & $19.09$                        & $16.92$                         & $16.22$                        & $20.27$                         & $18.55$                          & $17.20$                           & $18.56$                           & $18.53$                             \\ \cline{35-35} 
\end{tabular}
\end{table}

==> tables/lf_results.tex <==
\begin{table}[b]
    \centering
    \caption{Results for the action classifiers trained on Sims4Action~\cite{roitberg2021let} in the mPCA metric. The late fusion results are averaged over the $6$  fusion strategies discussed in Section \ref{sec:modality_extraction_and_training}. H: Heatmaps, L: Limbs, OF: Optical Flow.}
    \scalebox{0.75}{
    \begin{tabular}{l|ccc}
    \toprule
        {} & \multicolumn{3}{c}{mPCA [\%]} \\ \cline{2-4}
        {} & \multicolumn{1}{c}{\textsc{Synthetic}}& \multicolumn{2}{c}{\textsc{Real}} \\ \hline
        %
        
        \multicolumn{1}{r|}{Test Set}& \multirow{1}{*}{Sims4Action~\cite{roitberg2021let}} & \multirow{1}{*}{Toyota~\cite{das2019toyota}} & \multirow{1}{*}{ETRI~\cite{jang2020etri}} \\ \hline
        
        %
        \multicolumn{1}{l|}{Modalities} & {} & {} & {} \\ \hline
        

       % {} & {} & {} & {} & {} \\ \hline
         
         H & \multicolumn{1}{c}{$71.38$} & \multicolumn{1}{c}{$20.23$} & \multicolumn{1}{c}{$12.12$} \\
         %
         L & \multicolumn{1}{c}{$75.09$} & \multicolumn{1}{c}{$22.00$} & \multicolumn{1}{c}{$12.88$} \\
         %
         OF & \multicolumn{1}{c}{$44.50$} & \multicolumn{1}{c}{$21.34$} & 
         \multicolumn{1}{c}{$9.28$} \\
         %
         RGB & \multicolumn{1}{c}{$61.79$} & \multicolumn{1}{c}{$13.74$} & 
         \multicolumn{1}{c}{$9.37$}\\
         %
         YOLO & \multicolumn{1}{c}{$50.54$} & \multicolumn{1}{c}{$26.08$} & \multicolumn{1}{c}{$38.25$} \\ \hline
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L &  $91.48$  & $23.44$  & $16.95$ \\
         %
         H OF  & $89.86$  & $25.97$  & $15.10$ \\
         %
         H RGB  & $94.44$  & $21.38$  & $13.91$ \\
         %
         L OF  & $90.84$  & $25.60$  & $15.90$ \\
         %
         L RGB  & $94.42$  & $20.58$  & $15.46$ \\
         %
         OF RGB  & $86.15$  & $18.50$ &  $12.85$ \\ 
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H YOLO  & $74.86$  & $25.51$  & $20.55$ \\
         %
         L YOLO  & $80.25$ & $24.77$  & $19.91$ \\
         %
         OF YOLO & $62.21$  & $27.56$  & $20.34$ \\
         %
         RGB YOLO  & $76.23$  & $17.29$  & $19.41$ \\ \hline
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L OF  & $94.03$  & $26.70$  & $17.26$ \\
         %
         H L RGB  & $95.72$  & $23.25$  & $15.78$ \\
         %
         H OF RGB & $95.41$  & $23.73$  & $13.79$ \\
         %
         L OF RGB  & $95.61$  & $24.09$  & $15.49$ \\ 
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L YOLO  & $86.57$ & $25.80$  & $20.46$ \\
         H OF YOLO &   $82.97$ &   $29.48$ &   $19.91$ \\
         H RGB YOLO &   $88.79$ &   $23.27$ &   $17.77$ \\
         L OF YOLO &   $86.31$ &   $28.51$ &   $20.68$ \\
         L RGB YOLO &   $90.59$ &   $23.29$ &   $19.09$ \\
         OF RGB YOLO &   $82.37$ &   $21.15$ &   $16.92$ \\ \hline
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L OF RGB  & $96.95$  &  $26.00$  & $16.22$ \\
         %
         H L OF YOLO &   $90.05$ &   $28.98$ &   $20.27$ \\
         %
         H L RGB YOLO &   $92.88$ &   $25.36$ &   $18.55$ \\
         %
         H OF RGB YOLO &   $91.14$ &   $26.10$ &   $17.20$ \\
         %
         L OF RGB YOLO &   $92.56$ &   $26.12$ &   $18.56$ \\ \hline
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H L OF RGB YOLO &   $94.27$ &   $27.52$ &   $18.53$ \\
         \bottomrule
    \end{tabular}
    }
    \label{tab:lf_results}
\end{table}

==> tables/notation_table.tex <==

\renewcommand{\arraystretch}{1.4}

\begin{table*}[b]
    \centering
        \caption{Notation table for the terms in our equations.}
    \scalebox{0.95}{
    \begin{tabular}{l|l}
    \toprule
        Term & Explanation \\ \hline
        $\mathcal{M}$ & Set of all modalities: $\{\text{H, L, OF, RGB, YOLO}\}$. \\
        
        $\mathcal{C}$ & Set of all modality combinations (power set $2^{\mathcal{M}}$), i.e., $\mathcal{C}:=\{C | C \subseteq \mathcal{M}\} \setminus \emptyset$ \\
        
        $m \in \mathcal{M}$ & Modality, e.g. H \\ 
        
        $C \in \mathcal{C}$ & Modality combination, e.g., $\{\text{H},\text{L}\}$ \\
        
        $f(m) \in \mathbb{R}$ & Contribution of modality $m$ on the test dataset \\
        
        $acc(C) \in [0,1]$ & Accuracy of multimodal classifier on the test dataset with late fusion modality combination $C\in \mathcal{C}$ \\
        
        $\mathcal{M}^+ \subseteq \mathcal{M}$ & Modalities with a positive contribution, i.e. $\mathcal{M}^+ := \{m \in \mathcal{M} | f(m) > 0\}$ \\
        
        $\mathcal{M}^-\subseteq \mathcal{M}$ & Modalities with a negative contribution, i.e. $\mathcal{M}^- := \mathcal{M} \setminus \mathcal{M}^+$ and $\mathcal{M}^+ \cap \mathcal{M}^- = \emptyset$\\
        
        $AC_m$ & Unimodal action classifier trained on modality $m$ \\
        
       
        
        $\textbf{z}_m \in \mathbb{R}^N$ & Softmax class scores of $AC_m$ \\ 
        
        $\boldsymbol{\mu}_m \in \mathbb{R}^N$ & Expected class scores $\mathbb{E}[\textbf{z}_m]$ \\
        
        $\boldsymbol{\sigma}_m \in \mathbb{R}^N$ & Standard deviation of class scores $\sqrt{\mathbb{E}[(\textbf{z}_m - \boldsymbol{\mu}_m)^2]}$ \\
        
        $N \in \mathbb{N}$ & Number of action classes. \\
        
        $\odot$ & Element-wise multiplication. \\
        
        $\textbf{h}_m \in \mathbb{R}^d$ & Embedding from second-to-last layer of $AC_m$ \\
        
        $d \in \mathbb{N}$ & Embedding size \\
        
        $\rho(m,n) \in [-1,1]$ & Correlation between the predictions of $AC_m$ and $AC_n$ \\
        
        $MMD(m, n) \in \mathbb{R}^+$ & Maximum Mean Discrepancy between the embeddings $\textbf{h}_m$ and $\textbf{h}_n$ of $AC_m$ and $AC_n$ \\ 
        
        $\rho(m) \in [-1,1]$ & Aggregated correlations for modality $m$ \\
        
        $MMD(m) \in \mathbb{R}^+$ & Aggregated MMD for modality $m$ \\
        
        $A_\rho$ & Set of all $\rho(m)$, i.e., $\{\rho(m) | m \in \mathcal{M}\}$ \\
        
        $A_{MMD}$ & Set of all $MMD(m)$, i.e., $\{MMD(m) | m \in \mathcal{M}\}$ \\
        
        $\delta_{\textbf{agg}}^{\rho},\delta_{\textbf{agg}}^{MMD}$ & Aggregated thresholds for $A_\rho$ and $A_{MMD}$ \\
        
        $\mathcal{M}_{\textbf{agg}} \subseteq \mathcal{M}$ & Selected modalities from the consensus of $\delta_{\textbf{agg}}^{\rho}$ and $\delta_{\textbf{agg}}^{MMD}$ \\
        
        $\delta_{\textbf{pair}}^{\rho},\delta_{\textbf{pair}}^{MMD}$ & Pairs-thresholds for $\{\rho(m,n) | (m,n) \in \mathcal{M}^2\}$ and $\{MMD(m,n) | (m,n) \in \mathcal{M}^2\}$ \\
        
        $\mathcal{C}_{\textbf{pair}} \subseteq \mathcal{M}^2$ & Selected modality pairs from the consensus of $\delta_{\textbf{pair}}^{\rho}$ and $\delta_{\textbf{pair}}^{MMD}$ \\
        
        $sort(A)$ & Set $A$ sorted in ascending order $\{a_1,..a_{|A|} | a_i < a_{i+1}, \forall i \in \{1..|A|\}\}$ \\
        
        $\mu_{\lambda}(A)$ & $\lambda$-Winsorized Mean over the set $A$ \\
        
        $\lambda \in [0, 0.5]$ & Trust hyperparameter for $\mu_{\lambda}(\cdot)$ \\
        
        $a_\lambda$ & $\lambda$-percentile over a set $A$ \\
        
        $\bar{a}_\lambda$ & $\lambda$-trimmed mean over a set $A$, i.e., $\displaystyle \frac{1}{|A| - 2\lambda \cdot |A|} \cdot \sum_{i=\left\lceil \lambda \cdot |A| \right\rceil} ^ {|A| - \left\lceil \lambda \cdot |A| \right\rceil} sort(A)[i]$ \\
        
        
        
        
        
        

    
    \bottomrule
    \end{tabular}}
    
    \label{tab:notation_table}
\end{table*}
\clearpage

==> tables/selected_modalities.tex <==
\begin{table}[h]
    \centering
    \caption{Results from ModSelect: Selected modalities $\mathcal{M}_{\textbf{agg}}$ with $\delta_{\textbf{agg}}$ and selected modality pairs $\mathcal{C}_{\textbf{pair}}$ with $\delta_{\textbf{pair}}$ computed with Equations~\ref{eq:aggregated_consensus} and~\ref{eq:holistic_consensus}.}
    \label{tab:selected_modalities}
    \scalebox{0.75}{
    \begin{tabular}{l|c|c}
    \toprule
        Test Dataset & $\mathcal{M}_{\textbf{agg}}$ & $\mathcal{C}_{\textbf{pair}}$ \\ \hline 
        Sims4Action~\cite{roitberg2021let} & 
        \{H, L, RGB\} & \multirow{3}{*}{$\{(m,n) \in \mathcal{M}^2 | m \in \mathcal{M}^+ \land n \in \mathcal{M}^+\}$
        } \\ 
        Toyota~\cite{das2019toyota} & \{H, L, OF, YOLO\} & {} \\ 
        ETRI~\cite{jang2020etri} & \{H, L, YOLO\} & {} \\ 
        \bottomrule
    \end{tabular}}
    \vspace*{-1cm}
\end{table}

==> tables/yolo_table.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|c|c|c}
    \toprule
         Modalities & Sims & Toyota & ETRI  \\ \hline
         H & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         L & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         OF & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         RGB & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         YOLO & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         H+L & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         H+OF & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         H+RGB & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         L+OF & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         L+RGB & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         OF+RGB & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         H+L+OF & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         H+L+RGB & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         H+OF+RGB& $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         L+OF+RGB& $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         H+L+OF+RGB & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ & $\sim$ \\
         \bottomrule
    \end{tabular}
    \caption{TODO: Results from the multimodal S3D models trained on Sims4Action.}
    \label{tab:my_label}
\end{table}
